Sketched Reality: Sketching Bi-Directional Interactions Between Virtual and Physical Worlds with AR and Actuated Tangible UI

This paper introduces Sketched Reality, an approach that combines AR sketching and actuated tangible user interfaces (TUI) for bidirectional sketching interaction. Bi-directional sketching enables virtual sketches and physical objects to "affect" each other through physical actuation and digital computation. In the existing AR sketching, the relationship between virtual and physical worlds is only one-directional -- while physical interaction can affect virtual sketches, virtual sketches have no return effect on the physical objects or environment. In contrast, bi-directional sketching interaction allows the seamless coupling between sketches and actuated TUIs. In this paper, we employ tabletop-size small robots (Sony Toio) and an iPad-based AR sketching tool to demonstrate the concept. In our system, virtual sketches drawn and simulated on an iPad (e.g., lines, walls, pendulums, and springs) can move, actuate, collide, and constrain physical Toio robots, as if virtual sketches and the physical objects exist in the same space through seamless coupling between AR and robot motion. This paper contributes a set of novel interactions and a design space of bi-directional AR sketching. We demonstrate a series of potential applications, such as tangible physics education, explorable mechanism, tangible gaming for children, and in-situ robot programming via sketching.

==> alttext.tex <==
Figure 1.
Figure 1 shows one of the examples of Sketched Reality, a spring shot. Five photos taken from pull angle line up according to the procedure of the spring shot example. 
1. The left side shows the starting sketching with an iPad and a pen tool.
2. The middle left photo shows sketching a virtual spring line to the physical robot. 
3. The middle one shows a pulling physical robot with a virtual spring. 
4. The middle right photo shows the physical robot as spring shotted object to a virtual triangle lined with six balls. 
5. The right-side photo shows the end of the spring shot example flow. The physical robot collides with the virtual six balls, and bolls spread.


Figure 2.
Figure 2 illustrates the comparison of existing AR tools such as Reality Sketch, that physical object affects virtual object (left side), and our focus, Sketched Reality, that the virtual object affects physical object using an example of the collided virtual ball then the angle of the position relationship between physical robots change (right side).


Figure 3.
Figure 3 illustrates the design space for bi-directional interaction, including two comparing categories, Physical -> Virtual and Virtual -> Physical, in categories of four types of design space, boundary constraint, geometric constraint, applied force, and dynamic collision.


Figure 4.
Figure 4 is an illustration to represent the setup overview of our system. A person is sketching a virtual object using an iPad in the foreground, and a person is operating a physical robot in the background.


Figure 5.
Figure 5 shows the first step of the interaction flow of our system with three-lined screenshots, including supporting illustrations.
1. Left photo shows the set center point of the virtual canvas using the pen tool.
2. Middle photo shows the sketching of the virtual ball object using a pen tool.
3. Right photo shows the sketching line-based constraint to the sketched virtual ball. 


Figure 6.
Figure 6 shows the second step of the interaction flow of our system with three-lined screenshots supporting illustrations.
1. Left photo shows the sketching rectangle using a pen tool to set the stand.
2. Middle photo shows the sketched virtual rectangle and pendulum.
3. Right photo shows the setting status of the sketched rectangle as static by pen tapping.


Figure 7.
Figure 7 shows the third step of the interaction flow of our system with three-lined screenshots with supporting illustrations.
1. Left photo shows the scene of putting a physical robot on the mat.
2. Middle photo shows the setting status of the physical robot as adding gravity by pen tapping.
3. The right photo shows the physical robot releasing and colliding with the virtual rectangle object. 


Figure 8.
Figure 8 shows our system's four-step interaction flow with three-lined photos with supporting illustrations.
1. Left photo shows the scene of the setting the properties of a virtual pendulum with a pen touching
2. Middle photo shows the colliding of the pendulum with the physical robot.
3. Right one shows the result of the collision between the virtual pendulum and the physical robot.


Figure 9.
Figure 9 illustrates the application sketches using iPad scenarios categorized into four categories: Physical Education, Explorable Mechanism, Tangible Gaming, and In-situ Programming. This illustration shows two sketches for every four categories.
1. For physics education, shows Rube Goldberg Machine and Newton's Cradle.
2. For Explorable Mechanism, it shows Scissors Grab and Mechanical Piston.
3. For Tangible Gaming shows Pinball games and Hockey games.
4. For In-situ Programming, it shows In-situ Actuated TUI and Programming Motion by Sketching.


Figure 10.
Figure 10 shows one application - Rube Goldberg Machine with two slopes to represent a physics education scenario using three-lined photos.
1. Left photo shows the scene of leasing a physical robot to the first slope.
2. Middle photo shows the scene of the colliding of the physical robot with the virtual ball.
3. Left photo shows the scene of another colliding from the pushed virtual ball with another physical robot on the second slope.


Figure 11.
Figure 11 shows an application of Newton's Cradle to represent a physics education scenario using three-lined photos.
1. Left photo shows the scene of the released physical robot on the left side of Newton's Cradle.
2. Middle photo shows the scene of the physical robot colliding to line four virtual pendulums as middles of Newton's Cradle.
3. Right photo shows the virtual force propagation to the right-side physical robot.


Figure 12.
Figure 12 shows an application of the Piston Mechanism to represent a scenario using three-lined photos.
1. Left photo shows the left-hand grips of the physical robot connected with other physical robots through virtual line-shaped constraints.
2. Middle photo shows the left hand trying to circle the virtual circular constraint with holding the virtual robot as a kinetic element. Another physical robot on the road surrounded by two virtual rectangles is being pushed from virtual kinetic force progress from user manual movement.
3. Left photo shows the left hand trying to circle the virtual circular constraint with holding the virtual robot as a kinetic element. Another physical robot on the road surrounded by two virtual rectangles is being pulled from virtual kinetic force progress from user manual movement.


Figure 13.
Figure 13 shows an application of Pin Ball to represent a tangible gaming scenario using three-lined photos. 
1. Left photo shows that the user attacks the physical robot as a ball using the physical robot as an attack tool.
2. Middle photo shows that the virtually shot physical robot collides with the virtual wall.
3. Right photo shows the physical robot as the ball collides and bounds on the virtual wall and throws between virtual obstacle walls.

Figure 14.
Figure 14 shows an application of Pong to represent a tangible gaming scenario using three-lined photos.
1. Left photo shows that two players shot balls at each other using the physical robot as a shot tool. Left user shot 
2. Middle photo shows the virtual ball bounds the virtual wall, then the left user re-shot the virtual ball. Also, the shoot physical robot as the ball goes from left to right side.
3. The right photo shows the virtual shoot ball going through from left to right. Also, the right side user misses shooting the physical robot as the ball and fails the game. 


Figure 15.
Figure 15 shows an application of Actuated TUI control to represent an in-situ programming scenario using three-lined photos.
1. Left photo shows the start point of the scene where three robots as joints make a triangle shape each other, and the user holds the other physical robot as the control bar of the movement.
2. Middle photo shows that the user moves the physical robot as a control bar manually, then the shape-making robots start to move to change their position by changing the angle of the triangle.
3. The right photo shows that the user changes the angle of the triangle made with three physical robots using the physical robot as a control bar.


Figure 16.
Figure 16 shows an application of rope control to represent an in-situ programming scenario using three-lined photos.
1. Left photo shows three physical robots and the sketched virtual string.
2. Middle photo shows that the user controls the sketched virtual string with a pen tool from the iPad, then the three robots start moving when the string collides.
3. Right photo shows that the user controls the physical robots using the virtual string. 
